Top-Down Partitioning for Efficient List-Wise Ranking

Large Language Models (LLMs) have significantly impacted many facets of natural language processing and information retrieval. Unlike previous encoder-based approaches, the enlarged context window of these generative models allows for ranking multiple documents at once, commonly called list-wise ranking. However, there are still limits to the number of documents that can be ranked in a single inference of the model, leading to the broad adoption of a sliding window approach to identify the k most relevant items in a ranked list. We argue that the sliding window approach is not well-suited for list-wise re-ranking because it (1) cannot be parallelized in its current form, (2) leads to redundant computational steps repeatedly re-scoring the best set of documents as it works its way up the initial ranking, and (3) prioritizes the lowest-ranked documents for scoring rather than the highest-ranked documents by taking a bottom-up approach. Motivated by these shortcomings and an initial study that shows list-wise rankers are biased towards relevant documents at the start of their context window, we propose a novel algorithm that partitions a ranking to depth k and processes documents top-down. Unlike sliding window approaches, our algorithm is inherently parallelizable due to the use of a pivot element, which can be compared to documents down to an arbitrary depth concurrently. In doing so, we reduce the number of expected inference calls by around 33% when ranking at depth 100 while matching the performance of prior approaches across multiple strong re-rankers.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> src/table/main.tex <==
\begin{table}[t]
\caption{Comparing `Single Window', `Sliding Window', and `TDPart' (ours) approaches on TREC Deep Learning benchmarks. We report TOST (p<0.05), equivalence to our approach denoted with \underline{underline}. We report mean inferences with the mean number of inferences run in parallel in parentheses.
}
\setlength{\tabcolsep}{1.2pt}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}llrrrrrrrrr@{\hspace{3mm}}rrrrrrrrr@{\hspace{3mm}}rrrrrrrrr@{}}
\toprule
& & \multicolumn{9}{c}{\textbf{SPLADE ++ ED}} & \multicolumn{9}{c}{\textbf{RetroMAE}} & \multicolumn{9}{c}{\textbf{BM25}} \\
\cmidrule(r){3-11}
\cmidrule(r){12-20}
\cmidrule(r){21-29}
& & \multicolumn{2}{c}{nDCG@1} & \multicolumn{2}{c}{nDCG@5} & \multicolumn{2}{c}{nDCG@10} & \multicolumn{2}{c}{P@10} &  & \multicolumn{2}{c}{nDCG@1} & \multicolumn{2}{c}{nDCG@5} & \multicolumn{2}{c}{nDCG@10} & \multicolumn{2}{c}{P@10} &  & \multicolumn{2}{c}{nDCG@1} & \multicolumn{2}{c}{nDCG@5} & \multicolumn{2}{c}{nDCG@10} & \multicolumn{2}{c}{P@10} &  \\
\cmidrule(r){3-11}
\cmidrule(r){12-20}
\cmidrule(r){21-29}
Model & Mode & DL19 & DL20 & DL19 & DL20 & DL19 & DL20 & DL19 & DL20 & N. Inf. & DL19 & DL20 & DL19 & DL20 & DL19 & DL20 & DL19 & DL20 &  N. Inf. & DL19 & DL20 & DL19 & DL20 & DL19 & DL20 & DL19 & DL20 &  N. Inf. \\
\cmidrule(r){1-2}
\cmidrule(r){3-11}
\cmidrule(r){12-20}
\cmidrule(r){21-29}
Oracle & Single & \underline{0.977} & \underline{1.000} & 0.936 & \underline{0.977} & 0.890 & 0.916 & 0.765 & 0.748 & 1.0 (1.0) & 0.953 & 0.981 & 0.925 & 0.934 & 0.863 & 0.874 & 0.749 & 0.696 & 1.0 (1.0)  & 0.907 & 0.935 & 0.823 & 0.811 & 0.719 & 0.715 & 0.560 & 0.489 & 1.0 (1.0) \\
Oracle & Sliding & \underline{0.984} & \underline{1.000} & \underline{0.972} & \underline{0.995} & \underline{0.957} & \underline{0.978} & \underline{0.872} & \underline{0.822} & 9.0 (1.0)  & \underline{0.992} & \underline{1.000} & \underline{0.968} & \underline{0.993} & \underline{0.948} & \underline{0.958} & \underline{0.863} & \underline{0.800} & 9.0 (1.0) & \underline{0.953} & \underline{0.981} & \underline{0.924} & \underline{0.928} & \underline{0.879} & \underline{0.880} & \underline{0.788} & \underline{0.702} & 8.9 (1.0) \\
Oracle & TDPart & 0.984 & 1.000 & 0.972 & 0.995 & 0.956 & 0.976 & 0.872 & 0.820 & 7.0 (5.0) & 0.992 & 1.000 & 0.967 & 0.993 & 0.945 & 0.958 & 0.853 & 0.800 & 7.1 (5.1)  & 0.946 & 0.981 & 0.913 & 0.925 & 0.858 & 0.872 & 0.765 & 0.687 & 7.4 (5.4) \\
\midrule
Zephyr & Single & \underline{0.849} & \underline{0.855} & \underline{0.808} & \underline{0.831} & \underline{0.777} & \underline{0.795} & \underline{0.672} & \underline{0.637} & 1.0 (1.0)  & \underline{0.810} & \underline{0.867} & \underline{0.792} & \underline{0.815} & \underline{0.758} & \underline{0.778} & 0.665 & \underline{0.607} & 1.0 (1.0) & 0.713 & 0.784 & 0.681 & 0.689 & 0.625 & 0.628 & 0.500 & 0.435 & 1.0 (1.0) \\
Zephyr & Sliding & \underline{0.849} & \underline{0.849} & \underline{0.791} & \underline{0.826} & \underline{0.777} & \underline{0.802} & \underline{0.691} & \underline{0.631} & 9.0 (1.0) & \underline{0.810} & \underline{0.867} & \underline{0.796} & \underline{0.818} & \underline{0.769} & \underline{0.785} & \underline{0.686} & \underline{0.607} & 9.0 (1.0) & 0.713 & \underline{0.846} & 0.715 & \underline{0.770} & 0.707 & \underline{0.722} & 0.637 & \underline{0.535} & 8.9 (1.0) \\
Zephyr & TDPart & 0.833 & 0.852 & 0.794 & 0.828 & 0.780 & 0.805 & 0.679 & 0.639 & 7.4 (5.4) & 0.826 & 0.864 & 0.797 & 0.814 & 0.771 & 0.788 & 0.686 & 0.619 & 7.2 (5.2) & 0.736 & 0.858 & 0.731 & 0.772 & 0.681 & 0.723 & 0.577 & 0.543 & 7.4 (5.4) \\
\midrule
LiT5 & Single & \underline{0.802} & \underline{0.827} & \underline{0.795} & \underline{0.797} & \underline{0.763} & \underline{0.763} & \underline{0.665} & \underline{0.598} & 1.0 (1.0) & 0.787 & \underline{0.858} & \underline{0.773} & \underline{0.776} & \underline{0.739} & \underline{0.748} & 0.653 & \underline{0.585} & 1.0 (1.0) & 0.748 & 0.799 & 0.685 & 0.678 & 0.626 & 0.604 & 0.507 & 0.413 & 1.0 (1.0) \\
LiT5 & Sliding & \underline{0.802} & \underline{0.818} & \underline{0.798} & \underline{0.771} & \underline{0.774} & \underline{0.763} & \underline{0.691} & \underline{0.600} & 9.0 (1.0) & 0.756 & \underline{0.855} & \underline{0.770} & \underline{0.781} & \underline{0.741} & \underline{0.750} & 0.665 & \underline{0.578} & 9.0 (1.0) & 0.787 & \underline{0.833} & 0.751 & \underline{0.735} & 0.723 & \underline{0.700} & 0.640 & 0.531 & 8.9 (1.0)  \\
LiT5 & TDPart & 0.787 & 0.827 & 0.795 & 0.791 & 0.766 & 0.768 & 0.684 & 0.604 & 6.3 (4.3) & 0.740 & 0.867 & 0.763 & 0.798 & 0.743 & 0.761 & 0.684 & 0.591 & 6.6 (4.6) & 0.787 & 0.836 & 0.724 & 0.746 & 0.687 & 0.679 & 0.593 & 0.489 & 5.9 (3.9) \\
\midrule
GPT 3.5 & Single & 0.833 & 0.787 & \underline{0.783} & \underline{0.775} & \underline{0.760} & \underline{0.752} & \underline{0.644} & 0.607 & 1.0 (1.0) & 0.841 & 0.827 & \underline{0.802} & 0.789 & \underline{0.741} & \underline{0.744} & 0.630 & \underline{0.576} & 1.0 (1.0) & 0.698 & 0.765 & 0.647 & 0.666 & 0.602 & 0.588 & 0.484 & 0.393 & 1.0 (1.0) \\
GPT 3.5 & Sliding & 0.837 & 0.781 & \underline{0.786} & 0.779 & \underline{0.754} & 0.766 & \underline{0.642} & 0.617 & 9.0 (1.0) & 0.802 & \underline{0.799} & 0.779 & \underline{0.752} & \underline{0.740} & \underline{0.727} & 0.649 & 0.561 & 9.0 (1.0) & 0.709 & 0.809 & 0.727 & \underline{0.704} & 0.686 & 0.654 & 0.588 & 0.480 & 8.9 (1.0) \\
GPT 3.5 & TDPart & 0.802 & 0.806 & 0.779 & 0.788 & 0.753 & 0.752 & 0.642 & 0.598 & 7.4 (5.4) & 0.837 & 0.796 & 0.787 & 0.758 & 0.736 & 0.739 & 0.637 & 0.578 & 7.2 (5.2) & 0.686 & 0.802 & 0.693 & 0.708 & 0.654 & 0.637 & 0.556 & 0.459 & 7.5 (5.5) \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main}
\end{table}
